Effective Lagrangians from functional matching

We briefly review a variant of functional matching to derive an Effective Field Theory (EFT) for heavy particles at the one-loop level in the top-down approach. The method integrates out heavy fields that correspond to mass eigenstates, i.e. after removing mixing effects by diagonalizing mass matrices. Tree- and loop-level effects are separated by employing the background-field method, hard and soft modes are separated with the use of the expansion by regions. The method is exemplified for the Higgs Singlet Extension of the Standard Model where the mass $M_\mathrm{H}$ of the additional Higgs boson is considered large, and the Higgs mixing angle $\alpha$ is assumed to scale like $1/M_\mathrm{H}$, in order to guarantee decoupling in the large-$M_\mathrm{H}$ limit. Our calculation is agnostic w.r.t. the type (SMEFT vs. HEFT) of the emerging EFT. Eventually the emerging EFT Lagrangian can be transformed into SMEFT form, but only at the cost of introducing fermionic EFT operators, although no such operators are directly generated upon solving the functional integral over the heavy Higgs field.

==> defs.tex <==
% hyphenation patterns
\hyphenation{brems-strah-lung coun-ter-terms La-gran-gi-an}

\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}
% Use this to access bbold's \mathbb{1} as \bbid
\newcommand{\bbid}{\mathbbold{1}}

%  Abbreviations and math space and characters
\RequirePackage{xspace}
\providecommand*\eg{e.g.\@\xspace}
\providecommand*\ie{i.e.\@\xspace}
\providecommand*\cf{cf.\@\xspace}
\providecommand*\etc{etc.\@\xspace}
\providecommand*\etal{et al.\@\xspace}

% roman letters for mathematical constants and operators
\providecommand{\rd}{\ensuremath{\mathrm{d}}}
\providecommand{\re}{\ensuremath{\mathrm{e}}}
\providecommand{\rE}{\ensuremath{\mathrm{E}}}
\providecommand{\ri}{\ensuremath{\mathrm{i}}}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}
\providecommand{\hc}{\ensuremath{\text{h.c.}}\xspace}

% mathematical objects
\def\limfunc#1{\mathop{\rm #1}}
\def\tr{\limfunc{tr}}
%\newcommand{\order}[1]{\ensuremath{\mathcal{O}{\left(#1\right)}}\xspace}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}{(#1)}}\xspace}
\let\gsim\gtrsim
\let\lsim\lesssim
\makeatletter
\def\asymp#1%
{\mathrel{\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}}}
%\newcommand{\dsl}[1]{\not \hspace{-0.7mm}#1}
\def\Nlim#1{\mathrel{\raisebox{-.4em}
{$\stackrel{\displaystyle\longrightarrow}{\scriptstyle#1}$}}}
\def\dsl{\mathpalette\make@slash}
\def\make@slash#1#2{\setbox\z@\hbox{$#1#2$}%
  \hbox to 0pt{\hss$#1/$\hss\kern-\wd0}\box0}
\makeatother
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\sumbar}{\mathop{\overline{\sum}}}

% new commands for cross referencing
\def\refeq#1{\mbox{(\ref{#1})}}
\def\reffi#1{\mbox{Figure~\ref{#1}}}
\def\reffis#1{\mbox{Figures~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
\def\refapps#1{\mbox{Apps.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

\def\nn{\nonumber}

% shorthand for environments
\newcommand\nl{\notag\\}
\newcommand*\beq{\begin{equation}}
\newcommand*\eeq{\end{equation}}
\newcommand*\beqar{\begin{eqnarray}}
\newcommand*\eeqar{\end{eqnarray}}
\newcommand*\barr{\begin{array}}
\newcommand*\earr{\end{array}}
\newcommand*\bfi{\begin{figure}}
\newcommand*\efi{\end{figure}}
\newcommand*\btab{\begin{table}}
\newcommand*\etab{\end{table}}
\newcommand*\bpm{\begin{pmatrix}}
\newcommand*\epm{\end{pmatrix}}

%Shorthands for Greek letters
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand\eps{\epsilon}
\newcommand\veps{\varepsilon}
\newcommand\la{\lambda}
\newcommand\om{\omega}
\newcommand{\si}{\sigma}
\newcommand{\De}{\Delta}
\newcommand{\Ga}{\Gamma}
\newcommand\La{\Lambda}
\newcommand{\Si}{\Sigma}

% Units
\providecommand*\USP{\,}
\newcommand*{\Unit}[2]{\ensuremath{#1\USP\text{#2}}}
\newcommand{\pba}{\unskip\,\mathrm{pb}}
\newcommand{\fb}{{\ensuremath\unskip\USP\text{fb}}\xspace}
\newcommand{\MeV}{\ensuremath{\unskip\USP\text{Me\kern -0.1em V}}\xspace}
\newcommand{\GeV}{\ensuremath{\unskip\USP\text{Ge\kern -0.1em V}}\xspace}
\newcommand{\TeV}{\ensuremath{\unskip\USP\text{Te\kern -0.1em V}}\xspace}

% delta function
\newcommand{\deuf}{{\de^{(4)}}}

% SM parameters
\newcommand{\GF}{\ensuremath{G_\mu}}
\newcommand{\rs}{{\mathrm{s}}}
\newcommand{\rw}{{\mathrm{w}}}
\newcommand{\sw}{s_{\rw}}
\newcommand{\cw}{c_{\rw}}
\newcommand{\gs}{\ensuremath{g_\mathrm{s}}\xspace}
\newcommand{\alphas}{\ensuremath{\alpha_\rs}\xspace}
\newcommand{\Dalphahad}{\ensuremath{\Delta\alpha^{(5)}_{\mathrm{had}}\xspace}}
\newcommand{\If}{\ensuremath {I_{\rw,\Pf}^3}}
\newcommand{\Qf}{\ensuremath {Q_\Pf}}
\newcommand{\Qq}{\ensuremath {Q_\Pq}}
\newcommand{\Ql}{\ensuremath {Q_\Pl}}
\newcommand{\Qt}{\ensuremath {Q_\Pt}}
\newcommand{\VKM}{\ensuremath {{V}}}
\newcommand{\CL}{C_{\rL}}
\newcommand{\CR}{C_{\rR}}
\newcommand{\NCf}{\mathswitch {N_{\mathrm{C}}^\Pf}}
\newcommand{\NCt}{\mathswitch {N_{\mathrm{C}}^\Pt}}
\newcommand{\NCl}{\mathswitch {N_{\mathrm{C}}^\Pl}}
\newcommand{\NCq}{\mathswitch {N_{\mathrm{C}}^\Pq}}
\newcommand{\alphams}{\hat{\alpha}}
\newcommand{\Zms}{\hat{Z}}
\newcommand{\ems}{\hat{e}}
\newcommand{\gms}{\hat{g}}
\newcommand{\swms}{\hat{s}_{\rw}}
\newcommand{\cwms}{\hat{c}_{\rw}}
\newcommand{\kappams}{\hat{\kappa}}

% Particles
\newcommand{\Pg}{\ensuremath{\mathrm{g}}\xspace}
\newcommand{\PA}{\ensuremath{\gamma}\xspace}
\newcommand{\PW}{\ensuremath{\text{W}}\xspace}
\newcommand{\PWp}{\ensuremath{\PW^+}\xspace}
\newcommand{\PWm}{\ensuremath{\PW^-}\xspace}
\newcommand{\PWpm}{\ensuremath{\PW^\pm}\xspace}
\newcommand{\PZ}{\ensuremath{\text{Z}}\xspace}
\newcommand{\Ph}{\ensuremath{\text{h}}\xspace}
\newcommand{\PH}{\ensuremath{\text{H}}\xspace}
\newcommand{\Pe}{\ensuremath{\text{e}}\xspace}
\newcommand{\Pep}{\ensuremath{\Pe^+}\xspace}
\newcommand{\Pem}{\ensuremath{\Pe^-}\xspace}
\newcommand{\Pm}{\ensuremath{\mu}\xspace}
\newcommand{\Pb}{\ensuremath{\text{b}}\xspace}
\newcommand{\Pt}{\ensuremath{\text{t}}\xspace}
\newcommand{\Pu}{\ensuremath{\text{u}}\xspace}
\newcommand{\Pd}{\ensuremath{\text{d}}\xspace}
\newcommand{\Ps}{\ensuremath{\text{s}}\xspace}
\newcommand{\Pc}{\ensuremath{\text{c}}\xspace}
\newcommand{\Pbj}{\ensuremath{\text{j_b}}\xspace}
\newcommand{\Pj}{\ensuremath{\text{j}}\xspace}
\newcommand{\Pp}{\ensuremath{\text{p}}\xspace}
\newcommand{\Pq}{\ensuremath{q}\xspace}
\newcommand{\Pl}{\ensuremath{l}\xspace}
\newcommand{\Pn}{\ensuremath{\nu}\xspace}
\newcommand{\Pne}{\ensuremath{\nu_{\Pe}}\xspace}
\newcommand{\Pf}{\ensuremath{f}\xspace}

% Particle masses and widths
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\newcommand{\MWOS}{\ensuremath{M_{\PW,\text{OS}}}\xspace}
\newcommand{\MZOS}{\ensuremath{M_{\PZ,\text{OS}}}\xspace}
\newcommand{\Ml}{\ensuremath{m_\Pl}\xspace}
\newcommand{\Me}{\ensuremath{m_\Pe}\xspace}
\newcommand{\MW}{\ensuremath{M_\PW}\xspace}
\newcommand{\MZ}{\ensuremath{M_\PZ}\xspace}
\newcommand{\Mh}{\ensuremath{M_\Ph}\xspace}
\newcommand{\MH}{\ensuremath{M_\PH}\xspace}
\newcommand{\Mt}{\ensuremath{m_\Pt}\xspace}
\newcommand{\Mb}{\ensuremath{m_\Pb}\xspace}
\newcommand{\Mf}{\ensuremath{m_\Pf}\xspace}
\newcommand{\Mq}{\ensuremath{m_\Pq}\xspace}
\newcommand{\MP}{\ensuremath{M_P}\xspace}
\newcommand{\GP}{\ensuremath{\Gamma_P}\xspace}
\newcommand{\MV}{\ensuremath{M_V}\xspace}
\newcommand{\GV}{\ensuremath{\Gamma_V}\xspace}
\newcommand{\MPOS}{\ensuremath{M_{P,\,\OS}}\xspace}
\newcommand{\GPOS}{\ensuremath{\Gamma_{P,\OS}}\xspace}
\newcommand{\MVOS}{\ensuremath{M_{V,\OS}}\xspace}
\newcommand{\GVOS}{\ensuremath{\Gamma_{V,\OS}}\xspace}

% Particle widths
\newcommand{\GWOS}{\ensuremath{\Gamma_\PW^\text{OS}}\xspace}
\newcommand{\GZOS}{\ensuremath{\Gamma_\PZ^\text{OS}}\xspace}
\newcommand{\GZ}{\ensuremath{\Gamma_\PZ}\xspace}
\newcommand{\GW}{\ensuremath{\Gamma_\PW}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_\PH}\xspace}
\newcommand{\Gt}{\ensuremath{\Gamma_\Pt}\xspace}

\newcommand{\ren}{\mathrm{R}}
\newcommand{\rRe}{\mathop{\widetilde{\mathrm{Re}}}\nolimits}
\newcommand{\muR}{\mu_\mathrm{R}}
\newcommand{\muF}{\mu_\mathrm{F}}
\newcommand{\muIR}{\mu_\mathrm{IR}}
\newcommand{\deltaDR}{\eps}
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\MR}{\mathrm{MR}}

% calligraphic symbols
\newcommand{\cA}{\ensuremath{\mathcal{A}}\xspace}
%\newcommand{\cB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\cC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\cI}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\cK}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\cL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\cM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\cN}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\cO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\cP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\cV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\cW}{\ensuremath{\mathcal{W}}\xspace}

\newcommand{\ord}{\mathswitch{{\cal{O}}}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}
\newcommand{\Oaa}{\mathswitch{{\cal{O}}(\alpha^2)}}
\newcommand{\Oaaa}{\mathswitch{{\cal{O}}(\alpha^3)}}

% roman symbols
\newcommand{\rc}{\ensuremath{\text{c}}\xspace}
\newcommand{\rT}{\ensuremath{\text{T}}\xspace}
\newcommand{\rL}{\ensuremath{\text{L}}\xspace}
\newcommand{\rR}{\ensuremath{\text{R}}\xspace}
\newcommand{\rS}{\ensuremath{\text{S}}\xspace}
\newcommand{\rA}{\ensuremath{\text{A}}\xspace}
\newcommand{\rV}{\ensuremath{\text{V}}\xspace}
\newcommand{\rr}{\ensuremath{\text{r}}\xspace}
\newcommand{\rl}{\ensuremath{\text{l}}\xspace}
\newcommand{\rB}{\ensuremath{\text{B}}\xspace}
\newcommand{\rI}{\ensuremath{\text{I}}\xspace}

\newcommand{\sv}{\ensuremath{\sl v}}

%acronyms
\newcommand{\OS}{{\mathrm{OS}}}
\newcommand{\SU}{{\mathrm{SU}}}
\newcommand{\U}{{\mathrm{U}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\GSW}{{\mathrm{GSW}}}
\newcommand{\eff}{{\mathrm{eff}}}
\newcommand{\SM}{{\mathrm{SM}}}
\newcommand{\BSM}{{\mathrm{BSM}}}
\newcommand{\SESM}{{\mathrm{SESM}}}
\newcommand{\SMEFT}{{\mathrm{SMEFT}}}
\newcommand{\nonSMEFT}{{\,\cancel{\text{SMEFT}}}}
\newcommand{\MSbar}{\ensuremath{\overline{{\text{MS}}\xspace}}}
\newcommand{\UV}{{\mathrm{UV}}}
\newcommand{\weak}{{\mathrm{weak}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\tree}{{\mathrm{tree}}}
\def\oneloop{\text{1-loop}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\collCT}{{\textrm{coll-ct}}}
\newcommand{\hard}{{\mathrm{hard}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\EPA}{{\mathrm{EPA}}}
\newcommand{\ISR}{{\mathrm{ISR}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\LL}{{\mathrm{LL}}}
\newcommand{\LO}{{\mathrm{LO}}}
\newcommand{\NLO}{{\mathrm{NLO}}}
\newcommand{\PAx}{{\mathrm{PA}}}
\newcommand{\EW}{{\mathrm{EW}}}
\newcommand{\ew}{{\mathrm{EW}}}
\newcommand{\nf}{{\mathrm{nf}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\trunc}{{\mathrm{trunc}}}
\newcommand{\sa}{s_\alpha}

%codes
\newcommand{\Collier}{{\sc Collier}\xspace}
\newcommand{\HAWKTwo}{{\sc Hawk~2.0}\xspace}
\newcommand{\Recola}{{\sc Recola}\xspace}
\newcommand{\RecolaTwo}{{\sc Recola2}\xspace}
\newcommand{\Prophecy}{{\sc Prophecy4f}\xspace}
\newcommand{\Openloops}{{\sc OpenLoops}\xspace}
\newcommand{\MGNLO}{{\sc MadGraph5\_aMC@NLO}\xspace}
\newcommand{\Gosam}{{\sc GoSam}\xspace}
\newcommand{\FORM}{{\sc FORM}\xspace}
\newcommand{\NLOX}{{\sc NLOX}\xspace}

\renewcommand{\L}{\mathcal{L}}

% SMEFT parameters
\newcommand{\Lop}{\mathcal{O}}
\newcommand{\Lcoeff}{C}

% new environments
\newenvironment{myenumerate}%
{\begin{enumerate}[label=(\alph*),leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=2pt plus 1pt minus 1pt,parsep=0pt]}%
{\end{enumerate}}
\newenvironment{myitemize}%
{\begin{itemize}[leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=2pt plus 1pt minus 1pt,parsep=0pt]}%
{\end{itemize}}
\newenvironment{myaitemize}%
{\begin{itemize}[leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=4pt plus 2pt minus 2pt,parsep=0pt]}%
{\end{itemize}}

% new paragraph
\makeatletter
\newcommand\myparagraph{\@startsection{paragraph}{3}{\z@}%
  {-10\p@ \@plus 6\p@ \@minus 3\p@}%
  {3\p@}%
  {\normalfont\itshape}%
}
\makeatother

\newcommand*{\doi}[1]{\href{http://dx.doi.org/#1}{doi: #1}}


